ZeroQuant(4+2): Redefining LLMs Quantization with a New FP6-Centric Strategy for Diverse Generative Tasks

This study examines 4-bit quantization methods like GPTQ in large language models (LLMs), highlighting GPTQ's overfitting and limited enhancement in Zero-Shot tasks. While prior works merely focusing on zero-shot measurement, we extend task scope to more generative categories such as code generation and abstractive summarization, in which we found that INT4 quantization can significantly underperform. However, simply shifting to higher precision formats like FP6 has been particularly challenging, thus overlooked, due to poor performance caused by the lack of sophisticated integration and system acceleration strategies on current AI hardware. Our results show that FP6, even with a coarse-grain quantization scheme, performs robustly across various algorithms and tasks, demonstrating its superiority in accuracy and versatility. Notably, with the FP6 quantization, \codestar-15B model performs comparably to its FP16 counterpart in code generation, and for smaller models like the 406M it closely matches their baselines in summarization. Neither can be achieved by INT4. To better accommodate various AI hardware and achieve the best system performance, we propose a novel 4+2 design for FP6 to achieve similar latency to the state-of-the-art INT4 fine-grain quantization. With our design, FP6 can become a promising solution to the current 4-bit quantization methods used in LLMs.

==> _s6_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}


==> tables/alll_zeroshot.tex <==

\begin{table}[tb]
 \centering
 \caption{\textbf{Zero-Shot Evaluation (Perplexity).} Compare between GPTQ$_{C4}$ and RTN quantization algorithms for INT4 weight (W4A16) on \llama of size 1B, 13B and 65B. We apply  fine-grain quantization (FGQ) in which the block-size is 256 elements per scale (\llama-1B's block-size is 128). We also report results for coarse-grain quantization (CGQ) (per row per scale). The evaluation datasets are  Wikitext2, PTB, C4, PTB-new, and C4-new.} \label{table:ppl-all}
 \begin{adjustbox}{width=0.999\linewidth}\label{table:acc-int4}
\begin{tabular}{lllll}\toprule
 Precision &   FGQ    & \llama-1B (4096-seq)                                          & \llama-13B (2048-seq)                                     & \llama-65B (2048-seq)                                  \\\midrule
FP16    &  N/A & 24.31$_{7.53/37.39/8.91/58.34/9.40 }$      & 13.16$_{5.09/19.23/6.61/28.10/6.80 }$ & 6.41$_{3.56/8.00/5.62/8.88/5.98 }$  \\\midrule
INT4-GPTQ$_{C4}$  &  \cmark &564.73$_{7.83/1399.89/9.34/1396.76/9.84 }$ & 14.19$_{5.28/22.14/6.74/29.83/6.95}$  & 6.61$_{3.81/8.17/5.73/9.20/6.13 }$  \\
INT4-RTN   &  \cmark &22.76$_{7.98/34.03/9.50/52.28/10.00 }$     & 14.32$_{5.35/22.49/6.80/29.96/7.00 }$ & 7.30$_{3.79/10.13/5.74/10.54/6.31}$  \\
 INT4-GPTQ$_{C4}$  &  \xmark &288.22$_{8.20/719.21/9.84/693.48/10.37 }$  & 14.13$_{5.37/21.31/6.84/30.01/7.09 }$ & 7.17$_{4.12/10.50/5.83/9.16/6.21 }$ \\
 INT4-RTN   & \xmark & 34.29$_{8.33/55.52/10.15/86.85/10.62 }$    & 14.32$_{5.55/20.95/6.97/30.91/7.22 }$ & 7.72$_{4.20/10.59/5.90/11.44/6.47}$\\\midrule
  FP5-GPTQ$_{C4}$  &  \cmark & 44.29$_{7.74/72.63/9.19/122.20/9.68 }$ & 13.76$_{5.22/20.43/6.71/29.53/6.92 }$ &  6.50$_{3.67/8.15/5.68/8.95/6.04 }$\\
   FP5-RTN   &  \cmark &28.52$_{7.78/44.09/9.23/71.79/9.71 }$ & 13.95$_{5.20/21.01/6.71/29.92/6.92 }$&  6.83$_{3.70/9.73/5.69/8.98/6.06 }$\\
 \gb FP5-GPTQ$_{C4}$  &  \xmark &32.03$_{7.77/50.66/9.23/82.73/9.76 }$ &13.90$_{5.22/21.02/6.71/29.64/6.93 }$ &  6.46$_{3.68/7.83/5.70/9.13/5.98 }$\\
\gc FP5-RTN   &  \xmark  &27.92$_{7.83/41.80/9.27/70.94/9.77 }$ & 14.10$_{5.22/21.52/6.72/30.13/6.93 }$  &  6.50$_{3.68/8.08/5.69/8.98/6.06 }$\\  \midrule
FP6-GPTQ$_{C4}$  &  \cmark &22.77$_{7.59/34.04/8.98/53.76/9.47 }$ & 13.36$_{5.13/19.67/6.63/28.53/6.83 }$ & 6.47$_{3.59/8.12/5.63/8.91/6.10 }$ \\
FP6-RTN   &  \cmark &23.42$_{7.60/35.84/8.99/55.20/9.49 }$                                & 13.24$_{5.12/19.43/6.63/28.19/6.83 }$                                & 6.44$_{3.58/8.04/5.63/8.92/6.05 }$ \\  
\hb FP6-GPTQ$_{C4}$  &  \xmark &23.58$_{7.59/35.76/8.98/56.10/9.47 }$ & 13.23$_{5.12/19.34/6.64/28.20/6.83 }$ & 6.42$_{3.61/8.01/5.63/8.87/6.00 }$ \\
\hc FP6-RTN   &  \xmark &24.83$_{7.60/38.79/8.99/59.26/9.49 }$ & 13.09$_{5.12/19.06/6.64/27.81/6.83 }$ & 6.42$_{3.59/8.01/5.63/8.89/5.99 }$ \\  

\bottomrule  
\end{tabular}
\end{adjustbox}
 \end{table}


==> tables/old_table.tex <==
\begin{table}[H]
\caption{\textbf{Zero-shot Evaluation}. Compare FP6 and INT4 weight on \llama-13B (Top) and \llama-1B (Bottom) with per-row quantization using both GPTQ and RTN algorithms. \zhewei{Suggest to split the table to 2. It is too crowded. I change the order because: (1) normally, larger model comes later (as what you did for table 2. (2) better number comes later.}}\label{table:fp6-int6}
 \begin{adjustbox}{width=0.999\linewidth}
 \begin{tabular}{clccccccccccccc}\toprule 
&&& \multicolumn{1}{c}{Evaluation Perplexity} & \multicolumn{11}{c}{Zero-shot Evaluation (Metric: Accuracy)} \\
& Method                    & Precision     &  $\downarrow$ MEAN$_\text{(wiki/ptb/c4/ptb-new/c4-new)}$    &  arcC & arcE & boolq     & cb       & copa      & piqa     & rte       & wic      & wsc    & storyC  & $\uparrow$ MEAN  \\\midrule 
 &                         \multicolumn{3}{l}{\llama-1B (4096-seq)} \\
6&  N/A                             & FP16         & 24.31$_{7.53/37.39/8.91/58.34/9.40 }$     & 26.71          & 53.11     & 61.13 & 39.29     & 76.00    & 73.83     & 50.18    & 50.00     & 36.54    & 69.64       & 53.64  \\\cdashline{1-15}
7& \multirow{2}{*}{GPTQ$_\text{C4}$}     & INT4         & 288.22$_{8.20/719.21/9.84/693.48/10.37 }$ & 25.08          & 50.51     & 59.66 & 33.93     & 80.00    & 71.98     & 45.49    & 50.00     & 36.54    & 67.09       & 52.03  \\
8&        & \ourformat &  \textbf{23.58}$_{7.59/35.76/8.98/56.10/9.47 }$     & 26.37          & 52.53     & 61.19 & 42.86     & 75.00    & 73.50     & 51.26    & 50.00     & 36.54    & 69.76       &  \textbf{53.90}  \\\cdashline{1-15}
9& \multirow{2}{*}{Neareast}                & INT4         & 34.29$_{8.33/55.52/10.15/86.85/10.62 }$   & 28.75          & 50.80     & 57.03 & 35.71     & 76.00    & 71.76     & 51.26    & 49.84     & 36.54    & 69.89       & 52.76  \\
10&           & \ourformat &  \textbf{24.83}$_{7.60/38.79/8.99/59.26/9.49 }$     & 26.37          & 52.95     & 60.95 & 37.50     & 78.00    & 73.39     & 54.51    & 50.00     & 36.54    & 69.64       &  \textbf{53.99}  \\ 
\midrule
& \multicolumn{3}{l}{\llama-13B (2048-seq)} \\
1& N/A                      & FP16         & 13.16$_{5.09/19.23/6.61/28.10/6.80 }$     & 43.86          & 74.58     & 68.53 & 50.00     & 90.00    & 79.00     & 65.34    & 50.00     & 35.58    & 78.23       & 63.51  \\\cdashline{1-15}
2& \multirow{2}{*}{GPTQ}                 & INT4         & 14.13$_{5.37/21.31/6.84/30.01/7.09 }$     & 42.32          & 71.68     & 68.87 & 48.21     & 87.00    & 77.91     & 64.26    & 49.69     & 36.54    & 77.02       & 62.35  \\
3&            & \ourformat & \textbf{13.23}$_{5.12/19.34/6.64/28.20/6.83 }$     & 43.69          & 73.99     & 67.28 & 48.21     & 90.00    & 78.84     & 64.98    & 50.31     & 36.54    & 78.42       &  \textbf{63.23}  \\   \cdashline{1-15}
4& \multirow{2}{*}{Neareast}                    & INT4         & 14.32$_{5.55/20.95/6.97/30.91/7.22 }$     & 42.75          & 72.64     & 70.12 & 42.86     & 88.00    & 78.40     & 62.09    & 50.00     & 36.54    & 77.53       & 62.09  \\
5&        & \ourformat &  \textbf{13.09}$_{5.12/19.06/6.64/27.81/6.83 }$     & 43.77          & 74.20     & 68.38 & 46.43     & 91.00    & 78.84     & 65.34    & 49.84     & 36.54    & 78.23       &  \textbf{63.26}  \\
\bottomrule  
\end{tabular}
\end{adjustbox}
% \end{table}
% \begin{table}[H]
\caption{\textbf{Code Generation}. Compare FP6 and INT4 weight on \codegee-6B (Left) and \codestar-15B (Right) with per-row quantization using RTN algorithm.}
\begin{adjustbox}{width=0.999\linewidth}
\begin{tabular}{lc|cccc|cccc}\toprule 
  &              & \multicolumn{4}{c}{\codegee-6B}               & \multicolumn{4}{c}{\codestar-15B}               \\
  & Precision    & python     & cpp        & js         & MEAN    & python     & cpp        & js         & MEAN    \\\midrule 
1 & FP16         & 34.04$\pm$1.70  & 29.62$\pm$1.55 & 31.50$\pm$2.62  & 31.72 & 35.43$\pm$2.21 & 27.57$\pm$1.61 & 33.67$\pm$2.02 & 32.23 \\
3 & INT4         & 33.08$\pm$2.07 & 24.64$\pm$2.54 & 25.15$\pm$1.97 & 27.62 & 33.20$\pm$1.40   & 29.95$\pm$1.34 & 32.18$\pm$1.29 & 31.78 \\
2 & \ourformat & 34.10$\pm$2.09  & 27.74$\pm$1.18 & 31.61$\pm$1.74 & 31.15 & 35.64$\pm$1.26 & 27.91$\pm$1.49 & 33.60$\pm$1.91  & 32.38 \\
\bottomrule 
\end{tabular}
\end{adjustbox}
% \end{table}

% \begin{table}[H]
\caption{\textbf{Abstractive Summarization}. Compare FP6 and INT4 weight on BART-406M for the two datasets: CNN (Left) and XSUM (Right), with per-row quantization using RTN algorithm.}
\begin{adjustbox}{width=0.999\linewidth}
\begin{tabular}{lc|cccc|cccc}\toprule 
  &         & \multicolumn{4}{c}{\bart-CNN} & \multicolumn{4}{c}{\bart-XSUM} \\
  &         & Rouge-1  & Rouge-2  & Rouge-L  & Rouge-Lsum  & Rouge-1   & Rouge-2  & Rouge-L  & Rouge-Lsum  \\\midrule 
1 &  FP16       & 44.07   & 21.09   & 30.65   & 41.02      & 45.49    & 22.39   & 37.28   & 37.28      \\
3 & INT4     & 43.67   & 20.68   & 30.07   & 40.62      & 43.76    & 20.76   & 35.82   & 35.82  \\ 
2 & \ourformat & 44.06   & 21.07   & 30.67   & 40.99      & 45.37    & 22.20   & 37.11   & 37.11      \\
\bottomrule 
\end{tabular}
\end{adjustbox}
\end{table}

